Revisiting Hotels-50K and Hotel-ID

In this paper, we propose revisited versions for two recent hotel recognition datasets: Hotels50K and Hotel-ID. The revisited versions provide evaluation setups with different levels of difficulty to better align with the intended real-world application, i.e. countering human trafficking. Real-world scenarios involve hotels and locations that are not captured in the current data sets, therefore it is important to consider evaluation settings where classes are truly unseen. We test this setup using multiple state-of-the-art image retrieval models and show that as expected, the models' performances decrease as the evaluation gets closer to the real-world unseen settings. The rankings of the best performing models also change across the different evaluation settings, which further motivates using the proposed revisited datasets.

==> imgs/barplot_hotelid_rat1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.96\linewidth]{imgs/barplot_hotelid_rat1_pdf.pdf}
    \caption{\recallatone scores on \hotelsid.}
    \label{fig:hotelid-auc-barplot}
\end{figure}

==> imgs/barplot_hotels50k_rat1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.96\linewidth]{imgs/barplot_hotels50k_rat1_pdf.pdf}
    \caption{\recallatone scores on \hotelsfifty.}
    \label{fig:hotels50k-auc-barplot}
\end{figure}

==> imgs/fig1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{imgs/fig1_pdf.pdf}
    \caption{Images from the same hotel may (left) or may not (right) be connected, while images from different hotels may be connected (middle). Here, we have example images from four different hotels. Images from the same hotel are indicated with the same border color. We see that not all of the images in the same class are connected to each other (only purple class has all the pairwise connections between the examples). We also see that different classes can be connected to each other due to similar features (e.g., red and green class which share the same carpet).}
    \label{fig:image-linking}
\end{figure*}

==> imgs/img-hotels-examples.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imgs/img-hotels-examples_pdf.pdf}
    \caption{Examples of hotel images from three branches (classes) in the Hotels-50K and Hotel-ID datasets.}
    \label{fig:hotel-examples}
\end{figure}

==> sections/080listOfToDo.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\todototoc
\listoftodos

\textcolor{red}{LIST OF TODO}:

Camera version:
\begin{itemize}


    
\item training with random seeds two see which ones perform better
\item evaluating with multiple random seeds for an approximation and getting more robust results
\item training with multiple versions of splits with same characteristics

\item running multiple seeds for more robust experiments, 

\item fix model selection with two different model selection, one for auc one for image retrieval

\end{itemize}

Future: 
\begin{itemize}

\item Think of another domain for the dataset

\item Actually make a dataset with the characteristics we descirbe

\end{itemize}
